Question Decomposition with Dependency Graphs

QDMR is a meaning representation for complex questions, which decomposes questions into a sequence of atomic steps. While state-of-the-art QDMR parsers use the common sequence-to-sequence (seq2seq) approach, a QDMR structure fundamentally describes labeled relations between spans in the input question, and thus dependency-based approaches seem appropriate for this task. In this work, we present a QDMR parser that is based on dependency graphs (DGs), where nodes in the graph are words and edges describe logical relations that correspond to the different computation steps. We propose (a) a non-autoregressive graph parser, where all graph edges are computed simultaneously, and (b) a seq2seq parser that uses gold graph as auxiliary supervision. We find that a graph parser leads to a moderate reduction in performance (0.47 to 0.44), but to a 16x speed-up in inference time due to the non-autoregressive nature of the parser, and to improved sample complexity compared to a seq2seq model. Second, a seq2seq model trained with auxiliary graph supervision has better generalization to new domains compared to a seq2seq model, and also performs better on questions with long sequences of computation steps.

==> sections/appendices/error-analysis_bu.tex <==
\onecolumn
\subsection{Error Analysis Examples}
\label{apdx:error-analysis}

Table \ref{tab:error-analysis-examples} gives some examples for the error classes from \S\ref{sec:analysis:error-analysis}.

\begin{longtable}{lll}
% {l{0.2\textwidth}l{0.4\textwidth}l{0.4\textwidth}}
\small
% \begin{tabular}{lll}
                       & Gold                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & Prediction                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
Alternative Solutions & \begin{tabular}[c]{@{}l@{}}How many   yards longer was the longest field goal over the second longest?\\      1. select(sub=field goals)\\      2. project(projection=yards of \#REF; sub=\#1)\\      3. aggregate{[}max{]}(arg=longest \#2)\\      4. aggregate{[}max{]}(arg=second longest \#2)\\      5. arithmetic{[}difference{]}(left=\#3; right=\#4)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & \begin{tabular}[c]{@{}l@{}}CopyNet\\      1. select(sub=field goals)\\      2. project(projection=yards of \#REF; sub=\#1)\\      3. aggregate{[}max{]}(arg=\#2)\\      4. discard(exclude=\#3; sub=\#2)\\      5. aggregate{[}max{]}(arg=\#4)\\      6. arithmetic{[}difference{]}(left=\#3; right=\#5)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \cline{2-3} 
                      & \begin{tabular}[c]{@{}l@{}}If there   are exactly two fluffy dogs and no reflections.\\      1. select(sub=dogs)\\      2. filter(condition=that are fluffy; sub=\#1)\\      3. aggregate{[}count{]}(arg=\#2)\\      4. boolean{[}equals\_2{]}(condition=is equal to two; sub=\#3)\\      5. select(sub=reflections)\\      6. aggregate{[}count{]}(arg=\#5)\\      7. boolean{[}equals\_0{]}(condition=is equal to zero; sub=\#6)\\      8. boolean{[}logical\_and,true{]}(sub=\#4,\#7)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & \begin{tabular}[c]{@{}l@{}}Latent-RAT\\      1. select(sub=dogs)\\      2. filter(condition=that are fluffy; sub=\#1)\\      3. aggregate{[}count{]}(arg=\#2)\\      4. boolean{[}equals\_2{]}(condition=is equal to two; sub=\#3)\\      5. project(projection=reflections of \#REF; sub=\#2)\\      6. aggregate{[}count{]}(arg=\#5)\\      7. boolean{[}equals\_0{]}(condition=is equal to zero; sub=\#6)\\      8. boolean{[}logical\_and,true{]}(sub=\#4,\#7)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
Elaboration Level     & \begin{tabular}[c]{@{}l@{}}What tv   program with more than 19 episodes did Joey Lawrence play on?\\      1. select(sub=Joey Lawrence)\\      2. project(projection=tv programs of \#REF; sub=\#1)\\      3. filter(condition=with more than 19 episodes; sub=\#2)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}BiaffineGP\\      1. select(sub=Joey Lawrence)\\      2. project(projection=tv program; sub=\#1)\\      3. project(projection=episodes; sub=\#2)\\      4. group{[}count{]}(key=\#2; value=\#3)\\      5. comparative{[}more{]}(attribute=\#4; condition=more than 19; sub=\#2)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
Redundancy            & \begin{tabular}[c]{@{}l@{}}How many   TD passes were under 10 yards?\\      1. select(sub=TD passes)\\      2. project(projection=yards of \#REF; sub=\#1)\\      3. comparative{[}less{]}(attribute=\#2; condition=is lower than 10 yards;   sub=\#1)\\      4. aggregate{[}count{]}(arg=\#3)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}CopyNet\\      1. select(sub=TD passes)\\      2. project(projection=yards of \#REF; sub=\#1)\\      3. comparative{[}less{]}(attribute=\#2; condition=is lower than 10;   sub=\#1)\\      4. aggregate{[}count{]}(arg=\#3)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
Wrong Gold            & \begin{tabular}[c]{@{}l@{}}How many   objects are either yellow or shiny? \\      1. select(sub=objects)\\      2. filter(condition=that are yellow; sub=\#1)\\      3. filter(condition=that are shiny; sub=\#1)\\      4. aggregate{[}count{]}(arg=\#2)\\      5. aggregate{[}count{]}(arg=\#3)\\      6. arithmetic{[}sum{]}(arg=\#4,\#5)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}BiaffineGP\\      1. select(sub=objects)\\      2. filter(condition=shiny; sub=\#1)\\      3. discard(exclude=\#2; sub=\#1)\\      4. aggregate{[}count{]}(arg=\#2)\\      5. filter(condition=yellow; sub=\#3)\\      6. aggregate{[}count{]}(arg=\#5)\\      7. arithmetic{[}sum{]}(arg=\#4,\#6)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
Missing Information   & \begin{tabular}[c]{@{}l@{}}What shape   of the only object that wont roll if pushed?\\      1. select(sub=objects)\\      2. filter(condition=that wont roll if pushed; sub=\#1)\\      3. project(projection=shape of \#REF; sub=\#2)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \begin{tabular}[c]{@{}l@{}}CopyNet\\      1. select(sub=objects)\\      2. filter(condition=that has roll if pushed; sub=\#1)\\      3. project(projection=shape of \#REF; sub=\#2)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
Additional Steps      & \begin{tabular}[c]{@{}l@{}}What is   the smallestt shape and also yellow?\\      1. select(sub=shapes)\\      2. project(projection=size of \#REF; sub=\#1)\\      3. superlative{[}min{]}(attribute=\#2; sub=\#1)\\      4. filter(condition=that are yellow; sub=\#3)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}BiaffineGP\\      1. select(sub=shape)\\      2. comparative(condition=smallestt; sub=\#1)\\      3. project(projection=size; sub=\#1)\\      4. superlative{[}min{]}(attribute=\#3; sub=\#1)\\      5. filter(condition=yellow; sub=\#2,\#4)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
Additional Steps      & \begin{tabular}[c]{@{}l@{}}If at   least five orange dogs without collars sit upright in a row, gazing intently,   in one image, and the other image includes dogs in collars arranged more or   less in a row.\\      1. select(sub=one image)\\      2. project(projection=dogs in \#REF; sub=\#1)\\      3. filter(condition=that are orange; sub=\#2)\\      4. select(sub=collars)\\      5. filter(condition=\#4,without; sub=\#3)\\      6. filter(condition=that sit upright; sub=\#5)\\      7. filter(condition=in a row; sub=\#6)\\      8. filter(condition=that are gazing intently; sub=\#7)\\      9. aggregate{[}count{]}(arg=\#8)\\      10. boolean(condition=is at least five; sub=\#9)\\      11. select(sub=the other image)\\      12. project(projection=dogs in \#REF; sub=\#11)\\      13. filter(condition=\#4,in; sub=\#12)\\      14. boolean(condition=are arranged more or less in a row; sub=\#13)\\      15. boolean{[}logical\_and,true{]}(sub=\#10,\#14)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Latent-RAT\\      1. select(sub=one image)\\      2. project(projection=dogs in \#REF; sub=\#1)\\      3. filter(condition=that are orange; sub=\#2)\\      4. select(sub=collars)\\      5. filter(condition=that are orange; sub=\#3)\\      6. filter(condition=that are in a row; sub=\#5)\\      7. filter(condition=that are gazing intently; sub=\#6)\\      8. aggregate{[}count{]}(arg=\#7)\\      9. boolean(condition=is at least five; sub=\#8)\\      10. select(sub=other image)\\      11. project(projection=dogs in \#REF; sub=\#10)\\      12. project(projection=collars of \#REF; sub=\#10)\\      13. filter(condition=that are arranged more in a row; sub=\#12)\\      14. aggregate{[}count{]}(arg=\#13)\\      15. boolean(condition=is at least five; sub=\#14)\\      16. boolean{[}logical\_and,true{]}(sub=\#8,\#15)\end{tabular} \\ \hline
Wrong Logic           & \begin{tabular}[c]{@{}l@{}}How many   was the difference beween Sobieski's force and the Turks and Tatars?\\      1. select(sub=Sobieski)\\      2. project(projection=the force of \#REF; sub=\#1)\\      3. project(projection=size of \#REF; sub=\#2)\\      4. select(sub=the Turks and Tatars)\\      5. project(projection=the force of \#REF; sub=\#4)\\      6. project(projection=size of \#REF; sub=\#5)\\      7. arithmetic{[}difference{]}(left=\#6; right=\#3)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}Latent-RAT\\      1. select(sub=Sobieski)\\      2. project(projection=force of \#REF; sub=\#1)\\      3. select(sub=Turks)\\      4. select(sub=the Tatars)\\      5. arithmetic{[}difference{]}(left=\#2; right=\#3)\\      6. arithmetic{[}difference{]}(left=\#4; right=\#5)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \hline
Wrong Step Structure  & \begin{tabular}[c]{@{}l@{}}How many   years after Knopf was founded was it officiaully incorporated?\\      1. select(sub=Knopf was founded)\\      2. select(sub=Knopf was officiaully incorporated)\\      3. project(projection=year of \#REF; sub=\#1)\\      4. project(projection=year of \#REF; sub=\#2)\\      5. arithmetic{[}difference{]}(left=\#4; right=\#3)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & \begin{tabular}[c]{@{}l@{}}BiaffineGP\\      1. project(projection=Knopf was founded years; sub=\#1)\\      2. select(sub=was it officiaully incorporated)\\      3. project(projection=years; sub=\#2)\\      4. arithmetic{[}difference{]}(left=\#3; right=\#1)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \hline
Out of Vocab          & \begin{tabular}[c]{@{}l@{}}What   coutry is currently led by an acting prime minister and is a part of   NATO?\\      1. select(sub=NATO)\\      2. project(projection=coutries of \#REF; sub=\#1)\\      3. filter(condition=that are currently led by an acting prime minister;   sub=\#2)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}CopyNet\\      1. select(sub=company)\\      2. filter(condition=that is currently led by an acting prime minister;   sub=\#1)\\      3. filter(condition=that is part of NATO; sub=\#2)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
% \end{tabular}
\caption{
Error Classes Examples}
\label{tab:error-analysis-examples}
\end{longtable}

==> sections/appendices/eval-normalized-em.tex <==
\subsection{Rule-Based Evaluation (NormEM)}
\label{sec:eval-rule-based}
\todo{fill}

==> sections/appendices/graph_creation-tokens_alignment.tex <==
\subsection{ILP Based Token Alignment}
\label{sec:ILP-token-alignment}

Recall we denote by $q=\langle q_1, \dots ,q_n \rangle$ the question tokens and by $\forall i\in[1..m], s^i=s^i_1 \dots s^i_{n_i}$  the $i$th step tokens.  An \emph{alignment} is defined by $M=\{(q_i,s^k_j)\mid  q_i\approx s^k_j ;i\in[1..n], k\in[1..m], j\in[1..n_k] \}$, where by $t\approx t'$ we mean $t, t'$ are BREAK-equivalent (see Table \ref{tab:break-equivalance}). We say $t \sim_M t'$ iff $(t,t')\in M$ and $t_{1,\dots,d}\sim_M t_{1,\dots,d}$ iff $\forall i\in[1..d]: t_i\sim_M t'_i$. For readability we mostly omit the $M$ and just write $t \sim t'$ or $t_{1,\dots,d}\sim t'_{1,\dots,d}$ to mark that two tokens/sequences are aligned.

We can formalize the desired alignment restrictions (\S\ref{sec:graph-creation:tokens-alignment}) as an Integer Linear Program. For $i\in[1..n], k\in[1..m], j\in[1..n_k]$ let $x^k_{ij}\in\{0,1\}$ be an indicator for whether $(q_i,s^k_j)$ is in the output alignment, i.e $x^k_{ij} := \mathbbm{1}[(q_i,s^k_j)\in M]$. An assignment for these $\{x^k_{ij}\}$ binary variables defines a possible alignment.
\begin{equation}
    \forall i,j,k: x^k_{ij}\geq 0
\end{equation}
\begin{equation}
    \forall i,j,k: x^k_{ij}\leq 1
\end{equation}
\\

\paragraph{Validity} 
A valid alignment should align only equivalent tokens. Therefor, $x^k_{ij}$ can be $1$ just if $q_i \approx s^k_j$, otherwise it must be $0$. Let $a^k_{ij}\in\{0,1\}:=\mathbbm{1}[q_i \approx s^k_j]$ be an indicator for potential \emph{alignment}. We want to make sure that $a^k_{ij}=0 \Rightarrow x^k_{ij}=0$, so we restrict:
\begin{equation}
    \forall i,j,k: x^k_{ij}\leq a^k_{ij}
\end{equation}
\\

\paragraph{Exact Match} 
Similar to validity section, we define $b^k_{ij}\in\{0,1\}:=\mathbbm{1}[q_i = s^k_j]$ and would like to maximize:
\begin{equation}
    \max\sum_{k,i,j}b^{k}_{ij}x^{k}_{ij}
\end{equation}
\\

\paragraph{Steps Coverage} 
We would like each step token that has some potential question tokens to be aligned to at least one of them, i.e $\forall k,j: \lor_{i=1}^{n}a^k_{ij}\Rightarrow \lor_{i=1}^{n}x^k_{ij}$. Thus, we restrict
\begin{equation}
    \forall k,j: -\sum_{i=1}^{n}a^k_{ij} + n\sum_{i=1}^{n}x^k_{ij} \geq 0
\end{equation}
\\

\paragraph{Sequential Preference} 
We define auxiliary variables to maximize the length of aligned sequences. Let $y^{k,d}_{i,j}\in\{0,1\}, d\in\mathbbm{N}^+$ be an indicator for alignment of a sequence of length $d+1$ starting at $q_i, s^k_j$, i.e $y^{k,d}_{ij}:=\mathbbm{1}[q_{i,\dots,i+d} \sim s^k_{j,\dots,j+d}]$. Note $y^{k,d}_{ij} \iff \land_{p=0}^{d}x^k_{i+p,j+p} $, so we require:
\begin{equation}
    \forall d,k,i,j: -(d+1)y^{k,d}_{ij} + \sum_{p=0}^{d}x^k_{i+p, j+p} \geq 0
\end{equation}
\begin{equation}
    \forall d,k,i,j: y^{k,d}_{ij} - \sum_{p=0}^{d}x^k_{i+p, j+p} \geq -d
\end{equation}

We prefer long sequence alignment, meaning $\{y^k_{ij}\}$ with larger $d$'s to be $1$. We could define a monotonic scoring function that increases with $d$, $c(d):\mathbbm{N}^+\rightarrow \mathbbm{R}$ (e.g $c(d):=d$), and maximize $\sum_{d,k,i,j}c(d)y^{k,d}_{ij}$. However, since $y^{k,d}_{ij} \Rightarrow y^{k,d'}_{i'j'} \quad \forall d',i',j'\quad s.t \quad i\leq i', j \leq j', i'+d'\leq i+d, j'+d'\leq j+d$, we express this with:
\begin{equation}
    \max\sum_{d,k,i,j}y^{k,d}_{ij}
\end{equation}
\\


\paragraph{References Relations} 
Let $r^{k,k'}\in\{0,1\}$ indicate if step $k$ refers to step $k'$. We define auxiliaries variables that will help us count consecutive tokens in the question that are aligned to $k,k'$. $z^{+,k,k'}_i \iff (x^k_i \land r^{k,k'} \land x^{k'}_{i+1})$, $z^{-,k,k'}_i \iff (x^k_i \land r^{k,k'} \land x^{k'}_{i-1})$, where $x^k_i:= \lor_{j=1}^{n_k}x^k_{ij}$ (token $q_i$ is aligned to some token(s) of step $k$). We would like to maximize on $\{z^{+,k,k'},z^{-,k,k'}\}$:
\begin{equation}
    \forall k,i: -x^k_i+\sum_{j=1}^{n_k}x^k_{ij}\geq 0
\end{equation}
\begin{equation}
    \forall k,i: n_kx^k_i-\sum_{j=1}^{n_k}x^k_{ij}\geq 0
\end{equation}
\begin{equation}
    \forall k,k',i: -3z^{\pm,k,k'}_{i} + x^{k}_i + r^{k,k'} + x^{k'}_{i\pm1} \geq 0
\end{equation}
\begin{equation}
    \forall k,k',i: z^{\pm ,k,k'}_{i} - x^{k}_i - r^{k,k'} - x^{k'}_{i \pm 1} \geq -2
\end{equation}
\begin{equation}
    \max\sum_{k,k',i} z^{+ ,k,k'}_{i}+z^{- ,k,k'}_{i}
\end{equation}
\\


\paragraph{Minimalism} 
We want as few alignments as possible so intuitively we would like:
\begin{equation}
    \min\sum_{k,i,j}x^{k}_{ij}
\end{equation}
However, this constraint is not enough when there is a repeated question token/phrase that is aligned to more than one step. We would like each of the steps to be aligned to a separate copy of that phrase, i.e, each question token should be aligned to as few steps as possible, and ideally to a single \emph{unique} step. Let $u^{d}_{i}$ be an indicator for $q_i$ being aligned to at most $d \in \mathbbm{N}^+$ different steps, i.e, $u^d_i:=\mathbbm{1}(\exists K \subseteq [1..m], |K|\geq d: \forall k \in K, x^k_i=true)$. Intuitively, we want as few as possible such $u$'s for large $d$'s to be true. Since $\forall d,d', d \leq d' : u^{d'}_i \Rightarrow u^d_i$, it is enough to minimize over these $u$'s.
\begin{equation}
    \forall i,d: -du^d_i+\sum_{k}x^{k}_{i} \geq 0
\end{equation}
\begin{equation}
    \forall i,d: -mu^d_i + \sum_kx^k_i \leq d-1
\end{equation}
\begin{equation}
    \min\sum_{i,d}u^{d}_{i}
\end{equation}
\\

Eventually, our objective function is:\\
$
    \min\biggl[
    c_{min} \sum_{k,i,j}x^{k}_{ij} \\
    +c_{unique} \sum_{i,d}u^{d}_{i} \\
    -c_{exact} \sum_{k,i,j}b^{k}_{ij}x^{k}_{ij} \\
    -c_{seq} \sum_{d,k,i,j}y^{k,d}_{ij} \\
    -c_{ref} \sum_{k,k',i} (z^{+ ,k,k'}_{i}+z^{- ,k,k'}_{i})
    \biggr]
$ \\
Where we are taking $c_{min} \gg c_{unique} \gg c_{seq} \gg c_{exact}, c_{ref} $ to express the priorities between the preferences.


==> sections/appendices/graph_decoding.tex <==
\subsection{Dependency Graph Decoding}
\label{sec:gependencies-graph-decoding}
Our graph parser predicts probabilities over possible assignment of tags for every possible arc on top of the given tokens, but is not aware of any structural constraints during learning. We use a soft conversion into SDG in favor of evaluation and also provide an ILP-based post processing for fixing the produced probabilities according to the structural constraints.

\subsubsection{Soft Decoding}
Given a predicted DG we softly convert it into a SDG by first grouping the tokens into spans with respect to the \emph{span} dependencies. Two tokens are considered in the same span if there is an undirected path of \emph{span} dependencies between them. Doing so we allow no left-to-right \emph{span} dependencies, and multiple in/out \emph{span} dependencies to/from a single token. The dependencies between spans are induced by projecting their members' dependencies.
\subsubsection{ILP Based Decoding}
We formalize the DG specification to ILP constraints and solve an ILP with respect to the predicted probabilities.

Let $\mathcal{P} = \{p(i,j,t)\}$ be the predicted probabilities of a graph parser, where $\forall i,j \in [n], t \in Tags \cup \{none\}: p(i,j,t):=P[\textrm{the tag of arc (i,j) is t}]$. We would like to find a valid graph $G$ with maximal probability under $\mathcal{P}$ among the valid graphs. 

Denote $T := Tags$, $\bar{T} := T \cup \{none\}$. Let $x_{i,j,t}\in\{0,1\}$ be our target variables, i.e, $\forall i \in [n], j \in [n], t\in T,\ x_{i,j,t} := \mathbbm{1}[\textrm{the tag of arc (i,j) is t}]$. Note we omit $\{x_{i,j,none}\}$ to reduce the amount of variables, since $x_{i,j,none} = 1 - \sum_{t \in T}{x_{i,j,t}}$.

\paragraph{Maximal Probability} 
We would like our graph to maximize the probabilities given by $\mathcal{P}$, so our objective has to maximize:
\begin{equation}
\begin{split}
& \max \prod_{i,j;t\in \bar{T}} x_{i,j,t} p(i,j,t) = \\
& \max \sum_{i,j;t\in \bar{T}} x_{i,j,t} \log{p(i,j,t)} = \\
& \max \sum_{i,j;t\in T} x_{i,j,t} \log{p(i,j,t)} + \\ & \sum_{i,j} \left( 1- \sum_{t\in T}x_{i,j,t} \right) \log{\left( 1- \sum_{t\in T}p(i,j,t) \right)}
\end{split}
\end{equation}

\paragraph{Single Tag} 
We allow each arc to have a single tag only (or \emph{none}).
\begin{equation}
\forall i,j: \ \sum_{t\in T} x_{i,j,t} \leq 1
\end{equation}

\paragraph{Valid No-Operational Dependencies} 
\emph{span} and \emph{duplicate} have a specific roll which can be valid regardless of the other choices. \emph{span} is left-to-right, and \emph{duplicate} is from a \emph{[DUP]} token to a no-auxiliary token (\emph{[RSC], [DUP], [DUM]}). Let $a_{i,j,t} \in \{0,1\}$ be indicators for allowed tagging. We demand
\begin{equation}
\forall i,j,t \in T \ x_{i,j,t} \leq a_{i,j,t}
\end{equation}
And define $a_{i,j,t}$ to be $1$ except for the following cases
\begin{equation}
\forall i \geq j \ a_{i,j,span}=0
\end{equation}
\begin{multline}
\forall i,j: q_{i} \neq \text{[DUP]} \lor q_{j} \in \{\text{[RSC],[DUP],[DUM]}\} \\ \Rightarrow a_{i,j,duplicate}=0
\end{multline}
Moreover, each node can have at most a single incoming (outgoing) \emph{span} dependency, and at most a single outgoing \emph{duplicate}:
\begin{multline}
\forall i: \sum_{j} x_{i,j,span} \leq 1 \\ 
\forall j: \sum_{i} x_{i,j,span} \leq 1 \\
\forall i: \sum_{j} x_{i,j,duplicate} \leq 1 \\
\end{multline}
And finally, \emph{[DUP]} with some incoming/outgoing arcs must have an outgoing \emph{duplicate}, i.e, $\lor_{j, t}(x_{i,j,t} \lor x_{j,i,t}) \Rightarrow \lor_{j}x_{i,j,duplicate}$.
\begin{multline}
    \forall i, q_i=[DUP]: \\ -\sum\limits_{j,t}(x_{i,j,t}+x_{j,i,t})+2n|T|\sum\limits_{j}x_{i,j,duplicate} \geq 0
\end{multline}


\paragraph{Consistent Dependencies} 
Recall dependencies (tags) are given by triplets of the form $\langle operator, properties, arg \rangle$ (e.g $\text{filter-sub[equals]} = \langle filter, [equals], sub \rangle$). Since the outgoing arcs define a node operation we would like them to be consistent, i.e have the same \emph{operator} and \emph{properties}.

Let $\mathcal{O}$ be the possible operations and $Op:T \rightarrow \mathcal{O}$ a mapping from each tag (besides \emph{none}) to its operation. We define auxiliary variables $y_{i,o}^{out} \in \{0,1\}$ to indicates there is an outgoing arc from node $i$ with an operation $o$, and demand
\begin{equation}
\forall i  \ \sum_{o \neq duplicate} y_{i,o}^{out} \leq 1
\end{equation} 
More formally, $y_{i,o}^{out} := \mathbbm{1} \left[ \exists j \in [n], t \in T: x_{i,j,t}  \land Op(t)=o \right]$, and therefore $y_{i,o}^{out} = 1 \Leftrightarrow \sum_{j,t}x_{i,j,t}\mathbbm{1}\left[ Op(t)=o \right] \geq 1$. We obtain this by
\begin{multline}
\forall i, o \neq duplicate: \\ -\sum_{j,t}x_{i,j,t}\mathbbm{I}\left[ Op(t)=o \right] + n |T|y_{i,o}^{out} \geq 0
\end{multline} 
\begin{multline}
\forall i, o \neq duplicate:  \\ -y_{i,o}^{out} + \sum_{j,t}x_{i,j,t}\mathbbm{I}\left[ Op(t)=o \right] \geq 0
\end{multline} 

\paragraph{Span Single Representative} 
Recall a span is a left-to-right chain of \emph{span} arcs, where the rightmost token is used as the span representative. Each arc in/from this span should use the representative only. To achieve this, for each $j$ which is a non-representative node in a span chain, i.e, $y_{j,span}^{out} = 1$, we demand that $j$ will not have any incoming arcs but (maybe) a single \emph{span}, i.e $ \sum_{i,t\in T\setminus\{span\}}x_{i,j,t} \leq 0$ and $ \sum_{i}x_{i,j,span} \leq 1$.
\begin{multline}
\forall j:\\  \sum_{i,t\in T\setminus\{span\}}x_{i,j,t} + n(|T|-1)y_{j,span}^{out} \leq n(|T|-1)
\end{multline}
\begin{equation}
\forall j:  \sum_{i}x_{i,j,span} + ny_{j,span}^{out} \leq n + 1
\end{equation} 

\paragraph{Valid Dependency Combination} 
Operations sometimes induces constraints on dependency combinations. For example, \emph{union} must have at least two subjects; \emph{arithmetic-left} should be combined with \emph{arithmetic-right}, etc. Note that an argument might be ``missing'' (no outgoing dependency, no reference) if it's corresponding information is embedded in the span itself (e.g \emph{arithmetic[diff](left=\#1, right="100")}). If so, given a set of desired arguments we demand each of them has a corresponding arc pointing to a non-empty span, except (maybe) one if the current span is not empty.

We start by defining indicators for non-empty spans. First, mark no-empty tokens (s.a \emph{the, a, that, [RSC], [DUP], [DUM]}) using $m_{i}\in \{0,1\}$. Next, define $c_{i} \in \{0,1\}$ to be indicators for $q_{i}$ be a part of a content-holder (no-empty) span. We define $c_{i}$ in a recursive manner by $c_{i} \coloneqq m_i \lor \left( \lor_{k<i}(x_{k,i,span}\land c_{k}) \right) $ and if $q_i = \text{[DUP]}$ we add $\lor_{k<i}x_{i,k,duplicate}m_k$.

We add auxiliary variables $c_{k,i}:=x_{k,i,span} \land c_{k}$ and demand:
\begin{equation}
\begin{split}
\forall k \leq i: \\
2c_{k,i}-(x_{k,i,span}+c_k) \leq 0 \\
-c_{k,i}+(x_{k,i,span}+c_k) \leq 1
\end{split}
\end{equation}
\begin{equation}
\begin{split}
\forall i, q_i \neq \text{[DUP]}: \\
c_{0} := m_{0} \\
\sum_{k<i}c_{k,i}+m_{i}+(1-c_{i}) \geq 1 \\
-(\sum_{k<i}c_{k,i}+m_{i})+ic_{i} \geq 0
\end{split}
\end{equation}
\begin{equation}
\begin{split}
\forall i, q_i = \text{[DUP]}: \\
\sum_{k<i}c_{k,i}+\sum_{k<i}x_{i,k,dup}m_k+m_{i}+(1-c_{i}) \geq 1 \\
-(\sum_{k<i}c_{k,i}+\sum_{k<i}x_{i,k,dup}m_k+m_{i})+ic_{i} \geq 0
\end{split}
\end{equation}
Now, if we want a specific combination, $\tau=t_1, \dots , t_{|\tau|} \subseteq T$ to take place together (or not at all) we can demand $\sum_{t\in\tau}\bar{y}_{i,t}^{out}+c_i \geq |\tau|$ or $\sum_{t\in\tau}\bar{y}_{i,t}^{out} \leq 0$, where $\bar{y}^{out}_{i,t}$ are defined as $y^{out}_{i,o}$, but for full tags instead of just the operations. Let $z^{+}_{i,\tau}$, $z^{-}_{i,\tau}$ be indicators for these two conditions respectively. We want $z^{+}_{i,\tau} \lor z^{-}_{i,\tau}$ to hold.
\begin{equation}
\begin{split}
\forall i, \tau: \\
-|\tau|z^{-}_{i,\tau} + \sum_{t\in\tau}(1-\bar{y}^{out}_{i,t}) \geq |\tau| \\
-\sum_{t\in\tau}(1-\bar{y}^{out}_{i,t})+|\tau|z^{-}_{i,\tau} \geq 1-|\tau|
\end{split}
\end{equation}

\begin{equation}
\begin{split}
\forall i, \tau: \\
|\tau|(1-z^{+}_{i,\tau}) + \sum_{t\in\tau}\bar{y}^{out}_{i,t_h}+c_i \geq |\tau| \\
-2z^{+}_{i,\tau} +
\sum_{t\in\tau}\bar{y}^{out}_{i,t_h}+c_i < |\tau|
\end{split}
\end{equation}

\begin{equation}
    \forall i, \tau: z^{+}_{i,\tau} + z^{-}_{i,\tau} = 1
\end{equation}

Additional form of valid combinations constraint is $<\tau,\tau_{trigger}>$ where $\tau_{trigger} \subseteq \tau$ are dependencies that imply $\tau$, i.e, if one of $t_{i}, i \in \tau_{trigger}$, holds we want the entire $\tau$ to hold.

\paragraph{Connectivity}
Each QDMR step should be referred by other steps, except for the last step. Therefore, only a single span can have no incoming dependencies, i.e, be a \emph{root}. A \emph{root} (1) should have an outgoing dependency; (2) be a representative of a span (no outgoing \emph{span} dependency); (3) have no incoming dependency. 

Let $\{r_i\}_{i=1}^{n}$ be indicators for $q_i$ be a \emph{root}. We want $r_i \Leftrightarrow (1) \bigvee \limits_{j,t} x_{i,j,t} \lor \bigvee \limits_{k}x_{k,i,span}$ and $(2) \bigwedge \limits_{j} \lnot x_{i,j,span}$ and $(3) \bigwedge \limits_{k, t\neq span}\lnot x_{k,i,t}$, i.e $r_i=1 \Leftrightarrow \sum_{j,t}x_{i,j,t} + \sum_{k}x_{k,i,span} \geq 1 \land \sum_{k,t\neq span}x_{k,i,t} + \sum_{j}x_{i,j,span} \leq 0$. We demand
\begin{equation}
\begin{split}
    -r'_i + \sum_{j,t}x_{i,j,t} + \sum_{k}x_{k,i,span} \geq 0 \\
    -\sum_{j,t}x_{i,j,t} -\sum_{k}x_{k,i,span} + n(|T|+1)r'_i \geq 0
\end{split}
\end{equation}
\begin{equation}
\begin{split}
    -(1-r''_i) + \sum_{k,t\neq span}x_{k,i,t} + \sum_{j}x_{i,j,span} \geq 0 \\
    -\sum_{k,t\neq span}x_{k,i,t} - \sum_{j}x_{i,j,span} + n|T|(1-r''_i) \geq 0
\end{split}
\end{equation}
\begin{equation}
\begin{split}
    -2r_i+r'_i+r''_i \geq 0 \\
    -r'_i -r''_i +r_i \geq -1
\end{split}
\end{equation}
Finally we allow at most a single root
\begin{equation}
    \sum_{i}r_i \leq 1
\end{equation}

==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\commentout{
\paragraph{QDMR parsers}
As a new task, the majority work about QDMR parsing has given by \citet{wolfson2020break}. They supply a rule based model and a simple seq2seq LSTM-based model, where the best performances have reached by the CopyNet model \cite{Gu2016IncorporatingCM} - a seq2seq based model with a copy mechanism over the input tokens. 
% The encoder, a bi-directional RNN, is used to transform the source sequence into a series of hidden states. The decoder, an RNN that reads these hidden states and predicts the target sequence, uses attention mechanisms to produce a \emph{generate probabilities} over the vocabulary and \emph{copy probabilities} over the input sequence.

Note there were multiple submissions to AllenAI BREAK leaderboard\footnote{https://leaderboard.allenai.org/break/submissions/public}, but none of them has published yet. The top two models are based on BART \cite{lewis2019bart}, a denoising autoencoder for pretraining sequence-to-sequence models.
}

\paragraph{Semantic parsing} 
Forming dependency trees on top of an input sequence is a common technique in semantic parsing \cite{}.
Since 2014 \cite{oepen2015semeval}, a richer graph structured representation has used for dependency representations, allowing them to capture more linguistic information about a sentence in compare to the strict trees. Common approaches \cite{dozat2016deep, peng2017deep} involve bidirectional LSTM over word and part-of-speech tag embeddings followed by selfattention and an analgous multi-class classifier. Others \cite{wang2018neural} use a transition-based parser built on stack-LSTMs \cite{dyer2015transition}.
% first using a multilayer bidirectional LSTM
% over word and part-of-speech tag embeddings. Parsing is then done using directly-optimized selfattention over recurrent states to attend to each word’s head (or heads), and labeling is done with an analgous multi-class classifier.
% \citet{wang2018neural} use a transition-based parser built on stack-LSTMs \cite{dyer2015transition}. They extend \citet{choi2013transition} transition system for producing non-projective trees so that it can produce arbitrary DAGs.

\citet{dozat2018simpler} recently introduced a graph parser that is based on biaffine attention over tokens specification, factorized into two modules: one that predicts whether or not a directed edge exists between two tokens, and another that predicts the best label for each potential edge. 
% Both modules are based on bidirectional LSTM
% over word and part-of-speech tag embeddings. For each module, the encoddings are fed into two dedicated single-layer FFNs for head and dependent representation for each word. They then use bilinear or biaffine classifiers —which are generalizations of linear classifiers to include multiplicative interactions between two vectors—to predict edges and labels. 
More details are given in \S\ref{sec:models} as we use a variant of their model for predicting our graph representations.



\paragraph{RAT-SQL}
Various efforts have been taken for encoding schema into an input sequence \cite{guo2019towards, bogin2019representing}. Recently \citet{wang2019rat} present a unified framework, to address schema encoding, schema linking, and feature representation within a text-to-SQL
encoder, achieving the state-of-the-art on the Spider dataset \cite{yu2018spider}. RAT-SQL uses
relation-aware self-attention mechanism to combine global reasoning over the schema entities and question words with structured reasoning over predefined schema relations. The main idea is based on adding relative position information in a self-attention layer \cite{shaw2018self}, by using learned representations of the relationships between the input elements in the Transformer \cite{vaswani2017attention}.

In this work we use a variant of \emph{RAT-SQL}, the \textsc{Latent-RAT Encoder}, for encoding our QDMR-dependencies into the question. While \citet{shaw2018self} and \citet{wang2019rat} use known relations, we have no relations in advanced. Instead, we assume such relations are exist and retrieve their encodings based on a predecessors encoder for the RAT layers. We regularize these encoddings to represent a QDMR-dependency by additional classification layer on top of it, producing the desired dependency.

% Since our dependencies are declared for pairs of token, the mapping to $r_{ij}$ is quit straight forward. However, while \citet{shaw2018self} and \citet{wang2019rat} use known relations, in this work we have no relations in advanced. Instead, we assume such relations are exist and retrieve their encodings based on a predecessors encoder for the RAT layers. We regularize these encoddings to represent a QDMR-dependency by additional classification layer on top of it, producing the desired dependency. 

==> sections/related_work_bu.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{QDMR parsers}
As a new task, the majority work about QDMR parsing has given by \citet{wolfson2020break}. They supply a rule based model and a simple seq2seq LSTM-based model, where the best performances have reached by the CopyNet model \cite{Gu2016IncorporatingCM} - a seq2seq based model with a copy mechanism over the input tokens. The encoder, a bi-directional RNN, is used to transform the source sequence into a series of hidden states. The decoder, an RNN that reads these hidden states and predicts the target sequence, uses attention mechanisms to produce a \emph{generate probabilities} over the vocabulary and \emph{copy probabilities} over the input sequence.

Note there were multiple submissions to AllenAI BREAK leaderboard\footnote{https://leaderboard.allenai.org/break/submissions/public}, but none of them has published yet. The top two models are based on BART \cite{lewis2019bart}, a denoising autoencoder for pretraining sequence-to-sequence models.

\paragraph{Semantic parsing} 
Forming dependency trees on top of an input sequence is a common technique in semantic parsing \cite{}.
\todo{rephrase} The 2014 SemEval shared task on BroadCoverage Semantic Dependency Parsing  \cite{oepen2015semeval} introduced three new dependency representations that do away with the assumption of strict tree structure in favor of a richer graph structured representation, allowing them to capture more linguistic information about a sentence. 
In \citet{dozat2016deep} and \citet{peng2017deep}, parsing involves first using a multilayer bidirectional LSTM
over word and part-of-speech tag embeddings. Parsing is then done using directly-optimized selfattention over recurrent states to attend to each word’s head (or heads), and labeling is done with an analgous multi-class classifier.
\citet{wang2018neural} use a transition-based parser built on stack-LSTMs \cite{dyer2015transition}. They extend \citet{choi2013transition} transition system for producing non-projective trees so that it can produce arbitrary DAGs.

\citet{dozat2018simpler} recently introduced a graph parser that is based on biaffine attention over tokens specification, factorized into two modules: one that predicts whether or not a directed edge exists between two tokens, and another that predicts the best label for each potential edge. We briefly describe their model, as we will use it to examine our graph representation. They concatenate word and POS tag embeddings, and feed them into a multilayer bidirectional LSTM. For each of the two modules, they use single-layer feedforward networks (FNN) to split the top recurrent states into two parts—a head representation, as in Eq. (\ref{eq:graph-head}) and a dependent representation, as in Eq. (\ref{eq:graph-child}). They then use bilinear or biaffine classifiers in Eq. (\ref{eq:graph-biaffine})—which are generalizations of linear classifiers to include multiplicative interactions between two vectors—to predict edges and labels. 
The classifiers produce $n \times n$ and $n \times n \times |T|$ logits matrices correspondingly, where $n$ is the sequence length and $T$ is the tags set. The loss is the summation of the two cross entropy losses. On inference, the overall prediction is given by taking the tag with the maximal probability of arcs with $p_\textit{arc}$ greater from some threshold.

\begin{align}
& emb_i = emb^{word}_i \oplus emb^{POS}_i \nonumber \\ 
& e = \textit{BiLSTM}(emb) \in \mathbbm{R}^{n \times d}
\\
& r^\textit{arc-head}_i = \textit{FNN}^\textit{arc}_\textit{head}(e_i) \nonumber  \\
& r^\textit{tag-head}_i = \textit{FNN}^\textit{tag}_\textit{head}(e_i)  \label{eq:graph-head} \\
& r^\textit{arc-child}_i = \textit{FNN}^\textit{arc}_\textit{child}(e_i)
\nonumber \\
& r^\textit{tag-child}_i = \textit{FNN}^\textit{tag}_\textit{child}(e_i)
\label{eq:graph-child} \\
&S^\textit{arc} = [R^\textit{arc}_\textit{head}\ 1]W^\textit{arc} [R^\textit{arc}_\textit{child}\ 1]^T+b^\textit{arc} \nonumber \\
&S^\textit{tag} = R^\textit{tag}_\textit{head}W^\textit{tag} R^\textit{tag}_\textit{child}^T+b^\textit{tag} \label{eq:graph-biaffine}
\end{align}
Where $W^\textit{arc}\in \mathbbm{R}^{d+1 \times d+1}$, $W^\textit{tag}\in \mathbbm{R}^{d \times T \times d}$, $b^{arc}, b^{tag} \in \mathbbm{R}$ and $S^\textit{arc}\in\mathbbm{R}^{n \times n}$, $S^\textit{tag}\in\mathbbm{R}^{n \times n \times T}$. On inference:
\begin{equation*}
\small
  \begin{split}
&p^{arc}(i,j) = \sigma (S^\textit{arc}_{i,j})\\
&p^{tag}(i,j,t)=\textit{softmax}\limits_t S^\textit{tag}_{i,j,t}
\\
&y = \{(i,j,t) \mid p^{arc}(i,j) \geq 0.5, t=\textit{argmax}_{t} p^{tag}(i,j,t)\}
  \end{split}  
\end{equation*}



\paragraph{RAT-SQL}
Various efforts have been taken for encoding schema into an input sequence \cite{guo2019towards, bogin2019representing}. Recently \citet{wang2019rat} present a unified framework, to address schema encoding, schema linking, and feature representation within a text-to-SQL
encoder, achieving the state-of-the-art on the Spider dataset \cite{yu2018spider}. RAT-SQL uses
relation-aware self-attention mechanism to combine global reasoning over the schema entities and question words with structured reasoning over predefined schema relations. The main idea is based on adding relative position information in a self-attention layer \cite{shaw2018self} as follows:
\begin{equation}
\begin{split}
    e^{(h)}_{ij}&=\frac{x_iW^{(h)}_Q(x_jW^{(h)}_K+\textcolor{red}{r^K_{ij}})^T}{\sqrt{d_z/H}} \\
    z^{(h)}_i&=\sum_{j=1}^n{\alpha^{(h)}_{ij}(x_jW^{(h)}_V+\textcolor{red}{r^V_{ij}})}
\end{split}
\end{equation}

Where the $r_{ij}$ terms encode the relationship between the input elements $x_i, x_j$. The rest is the standard self-attention encoder, or Transformer \cite{vaswani2017attention}. \mh{elaborate?}
In this work we use a variant of \emph{RAT-SQL} for encoding our QDMR-dependencies into the question. Since our dependencies are declared for pairs of token, the mapping to $r_{ij}$ is quit straight forward. However, while \citet{shaw2018self} and \citet{wang2019rat} use known relations, in this work we have no relations in advanced. Instead, we assume such relations are exist and retrieve their encodings based on a predecessors encoder for the RAT layers. We regularize these encoddings to represent a QDMR-dependency by additional classification layer on top of it, producing the desired dependency. 
